ChatGPT vs State-of-the-Art Models: A Benchmarking Study in Keyphrase Generation Task

Transformer-based language models, including ChatGPT, have demonstrated exceptional performance in various natural language generation tasks. However, there has been limited research evaluating ChatGPT's keyphrase generation ability, which involves identifying informative phrases that accurately reflect a document's content. This study seeks to address this gap by comparing ChatGPT's keyphrase generation performance with state-of-the-art models, while also testing its potential as a solution for two significant challenges in the field: domain adaptation and keyphrase generation from long documents. We conducted experiments on six publicly available datasets from scientific articles and news domains, analyzing performance on both short and long documents. Our results show that ChatGPT outperforms current state-of-the-art models in all tested datasets and environments, generating high-quality keyphrases that adapt well to diverse domains and document lengths.

==> references.tex <==
@inproceedings{kp-class,
    title = "A Study on Automatically Extracted Keywords in Text Categorization",
    author = "Hulth, Anette  and
      Megyesi, Be{\'a}ta B.",
    booktitle = "Proceedings of the 21st International Conference on Computational Linguistics and 44th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2006",
    address = "Sydney, Australia",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/P06-1068",
    doi = "10.3115/1220175.1220243",
    pages = "537--544",
}

@InProceedings{kp-cluster,
author="Hammouda, Khaled M.
and Matute, Diego N.
and Kamel, Mohamed S.",
editor="Perner, Petra
and Imiya, Atsushi",
title="CorePhrase: Keyphrase Extraction for Document Clustering",
booktitle="Machine Learning and Data Mining in Pattern Recognition",
year="2005",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="265--274",
abstract="The ability to discover the topic of a large set of text documents using relevant keyphrases is usually regarded as a very tedious task if done by hand. Automatic keyphrase extraction from multi-document data sets or text clusters provides a very compact summary of the contents of the clusters, which often helps in locating information easily. We introduce an algorithm for topic discovery using keyphrase extraction from multi-document sets and clusters based on frequent and significant shared phrases between documents. The keyphrases extracted by the algorithm are highly accurate and fit the cluster topic. The algorithm is independent of the domain of the documents. Subjective as well as quantitative evaluation show that the algorithm outperforms keyword-based cluster-labeling algorithms, and is capable of accurately discovering the topic, and often ranking it in the top one or two extracted keyphrases.",
isbn="978-3-540-31891-0"
}

@inproceedings{kp-summarization,
    title = "Citation Summarization Through Keyphrase Extraction",
    author = {Qazvinian, Vahed  and
      Radev, Dragomir R.  and
      {\"O}zg{\"u}r, Arzucan},
    booktitle = "Proceedings of the 23rd International Conference on Computational Linguistics (Coling 2010)",
    month = aug,
    year = "2010",
    address = "Beijing, China",
    publisher = "Coling 2010 Organizing Committee",
    url = "https://aclanthology.org/C10-1101",
    pages = "895--903",
}

@misc{kp-recom,
      title={SemEval 2017 Task 10: ScienceIE - Extracting Keyphrases and Relations from Scientific Publications}, 
      author={Isabelle Augenstein and Mrinal Das and Sebastian Riedel and Lakshmi Vikraman and Andrew McCallum},
      year={2017},
      eprint={1704.02853},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@Article{kp-information-retrieval,
  author={Debarshi Kumar Sanyal and Plaban Kumar Bhowmick and Partha Pratim Das and Samiran Chattopadhyay and T. Y. S. S. Santosh},
  title={{Enhancing access to scholarly publications with surrogate resources}},
  journal={Scientometrics},
  year=2019,
  volume={121},
  number={2},
  pages={1129-1164},
  month={November},
  keywords={Scholarly publication; Open access; Academic search; Digital library; Approximate match},
  doi={10.1007/s11192-019-03227-},
  abstract={ Digital libraries containing scholarly publications are common today. They are an invaluable source of information to students, researchers, and practitioners. However, many digital libraries expose only the article metadata like title, author names, publication date, and the abstract for free; access to full-text requires access toll. Given that journal subscription charges are sometimes prohibitive, many important publications remain beyond the access of researchers, especially in developing countries. While open access publication solves this issue, the hard reality is that many research papers are not currently available for free reading or download. In this paper, we present a novel approach to alleviate this problem. We present a technique to retrieve open access surrogates of a scholarly article when the latter is unavailable freely in a digital library. Surrogates are articles semantically close to the original articles, written by the same author(s) and give valuable insights into the paper being searched for; they address the same or a very similar problem using the same or very similar techniques. Our focus on approximate matches of scholarly articles distinguishes our application from many academic search engines. We run it on a large corpus of computer science papers and compare the results with human judgment. Experimental results show that our tool can indeed identify relevant OA surrogates of access-restricted papers.},
  url={https://ideas.repec.org/a/spr/scient/v121y2019i2d10.1007_s11192-019-03227-4.html}
}

@inproceedings{sahrawat2020keyphrase,
  title={Keyphrase extraction as sequence labeling using contextualized embeddings},
  author={Sahrawat, Dhruva and Mahata, Debanjan and Zhang, Haimin and Kulkarni, Mayank and Sharma, Agniv and Gosangi, Rakesh and Stent, Amanda and Kumar, Yaman and Shah, Rajiv Ratn and Zimmermann, Roger},
  booktitle={European Conference on Information Retrieval},
  pages={328--335},
  year={2020},
  organization={Springer}
}

@article{transkp,
  title={TransKP: Transformer based Key-Phrase Extraction},
  author={Mukund Rungta and Rishabh Kumar and Mehak Preet Dhaliwal and Hemant Tiwari and Vanraj Vala},
  journal={2020 International Joint Conference on Neural Networks (IJCNN)},
  year={2020},
  pages={1-7}
}

@inproceedings{alzaidy_2019,
author = {Alzaidy, Rabah and Caragea, Cornelia and Giles, C. Lee},
title = {Bi-LSTM-CRF Sequence Labeling for Keyphrase Extraction from Scholarly Documents},
year = {2019},
isbn = {9781450366748},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3308558.3313642},
doi = {10.1145/3308558.3313642},
abstract = {In this paper, we address the keyphrase extraction problem as sequence labeling and propose a model that jointly exploits the complementary strengths of Conditional Random Fields that capture label dependencies through a transition parameter matrix consisting of the transition probabilities from one label to the neighboring label, and Bidirectional Long Short Term Memory networks that capture hidden semantics in text through the long distance dependencies. Our results on three datasets of scholarly documents show that the proposed model substantially outperforms strong baselines and previous approaches for keyphrase extraction.},
booktitle = {The World Wide Web Conference},
pages = {2551–2557},
numpages = {7},
keywords = {deep learning., Keyphrase extraction, sequence labeling},
location = {San Francisco, CA, USA},
series = {WWW '19}
}

@article{Gollapalli_Li_Yang_2017, 
title={Incorporating Expert Knowledge into Keyphrase Extraction}, volume={31}, url={https://ojs.aaai.org/index.php/AAAI/article/view/10986}, DOI={10.1609/aaai.v31i1.10986}, number={1}, journal={Proceedings of the AAAI Conference on Artificial Intelligence}, author={Gollapalli, Sujatha Das and Li, Xiao-li and Yang, Peng}, year={2017}, month={Feb.} }

@InProceedings{nguyen_kan_2007,
author="Nguyen, Thuy Dung
and Kan, Min-Yen",
editor="Goh, Dion Hoe-Lian
and Cao, Tru Hoang
and S{\o}lvberg, Ingeborg Torvik
and Rasmussen, Edie",
title="Keyphrase Extraction in Scientific Publications",
booktitle="Asian Digital Libraries. Looking Back 10 Years and Forging New Frontiers",
year="2007",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="317--326",
isbn="978-3-540-77094-7"
}

@inproceedings{keybart,
    title = "Learning Rich Representation of Keyphrases from Text",
    author = "Kulkarni, Mayank  and
      Mahata, Debanjan  and
      Arora, Ravneet  and
      Bhowmik, Rajarshi",
    booktitle = "Findings of the Association for Computational Linguistics: NAACL 2022",
    month = jul,
    year = "2022",
    address = "Seattle, United States",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.findings-naacl.67",
    doi = "10.18653/v1/2022.findings-naacl.67",
    pages = "891--906",
}

@misc{lewis2019bart,
      title={BART: Denoising Sequence-to-Sequence Pre-training for Natural Language Generation, Translation, and Comprehension}, 
      author={Mike Lewis and Yinhan Liu and Naman Goyal and Marjan Ghazvininejad and Abdelrahman Mohamed and Omer Levy and Ves Stoyanov and Luke Zettlemoyer},
      year={2019},
      eprint={1910.13461},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{raffel2020exploring,
      title={Exploring the Limits of Transfer Learning with a Unified Text-to-Text Transformer}, 
      author={Colin Raffel and Noam Shazeer and Adam Roberts and Katherine Lee and Sharan Narang and Michael Matena and Yanqi Zhou and Wei Li and Peter J. Liu},
      year={2020},
      eprint={1910.10683},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{Radford2018ImprovingLU,
  title={Improving Language Understanding by Generative Pre-Training},
  author={Alec Radford and Karthik Narasimhan},
  year={2018}
}

@inproceedings{Radford2019LanguageMA,
  title={Language Models are Unsupervised Multitask Learners},
  author={Alec Radford and Jeff Wu and Rewon Child and David Luan and Dario Amodei and Ilya Sutskever},
  year={2019}
}

@misc{brown2020language,
      title={Language Models are Few-Shot Learners}, 
      author={Tom B. Brown and Benjamin Mann and Nick Ryder and Melanie Subbiah and Jared Kaplan and Prafulla Dhariwal and Arvind Neelakantan and Pranav Shyam and Girish Sastry and Amanda Askell and Sandhini Agarwal and Ariel Herbert-Voss and Gretchen Krueger and Tom Henighan and Rewon Child and Aditya Ramesh and Daniel M. Ziegler and Jeffrey Wu and Clemens Winter and Christopher Hesse and Mark Chen and Eric Sigler and Mateusz Litwin and Scott Gray and Benjamin Chess and Jack Clark and Christopher Berner and Sam McCandlish and Alec Radford and Ilya Sutskever and Dario Amodei},
      year={2020},
      eprint={2005.14165},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{ouyang2022training,
      title={Training language models to follow instructions with human feedback}, 
      author={Long Ouyang and Jeff Wu and Xu Jiang and Diogo Almeida and Carroll L. Wainwright and Pamela Mishkin and Chong Zhang and Sandhini Agarwal and Katarina Slama and Alex Ray and John Schulman and Jacob Hilton and Fraser Kelton and Luke Miller and Maddie Simens and Amanda Askell and Peter Welinder and Paul Christiano and Jan Leike and Ryan Lowe},
      year={2022},
      eprint={2203.02155},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{textrank,
    title = "{T}ext{R}ank: Bringing Order into Text",
    author = "Mihalcea, Rada  and
      Tarau, Paul",
    booktitle = "Proceedings of the 2004 Conference on Empirical Methods in Natural Language Processing",
    month = jul,
    year = "2004",
    address = "Barcelona, Spain",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/W04-3252",
    pages = "404--411",
}

@inproceedings{topicrank,
    title = "{T}opic{R}ank: Graph-Based Topic Ranking for Keyphrase Extraction",
    author = "Bougouin, Adrien  and
      Boudin, Florian  and
      Daille, B{\'e}atrice",
    booktitle = "Proceedings of the Sixth International Joint Conference on Natural Language Processing",
    month = oct,
    year = "2013",
    address = "Nagoya, Japan",
    publisher = "Asian Federation of Natural Language Processing",
    url = "https://aclanthology.org/I13-1062",
    pages = "543--551",
}

@inproceedings{mahata2018key2vec,
  title={Key2vec: Automatic ranked keyphrase extraction from scientific articles using phrase embeddings},
  author={Mahata, Debanjan and Kuriakose, John and Shah, Rajiv and Zimmermann, Roger},
  booktitle={Proceedings of the 2018 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 2 (Short Papers)},
  pages={634--639},
  year={2018}
}

@inproceedings{wang2014corpus,
  title={Corpus-independent generic keyphrase extraction using word embedding vectors},
  author={Wang, Rui and Liu, Wei and McDonald, Chris},
  booktitle={Software engineering research conference},
  volume={39},
  pages={1--8},
  year={2014}
}

@article{bennani2018simple,
  title={Simple unsupervised keyphrase extraction using sentence embeddings},
  author={Bennani-Smires, Kamil and Musat, Claudiu and Hossmann, Andreea and Baeriswyl, Michael and Jaggi, Martin},
  journal={arXiv preprint arXiv:1801.04470},
  year={2018}
}

@inproceedings{hulth2003,
author = {Hulth, Anette},
title = {Improved Automatic Keyword Extraction given More Linguistic Knowledge},
year = {2003},
publisher = {Association for Computational Linguistics},
address = {USA},
url = {https://doi.org/10.3115/1119355.1119383},
doi = {10.3115/1119355.1119383},
booktitle = {Proceedings of the 2003 Conference on Empirical Methods in Natural Language Processing},
pages = {216–223},
numpages = {8},
series = {EMNLP '03}
}

@inproceedings{kim-kan-2009-examining,
    title = "Re-examining Automatic Keyphrase Extraction Approaches in Scientific Articles",
    author = "Kim, Su Nam  and
      Kan, Min-Yen",
    booktitle = "Proceedings of the Workshop on Multiword Expressions: Identification, Interpretation, Disambiguation and Applications ({MWE} 2009)",
    month = aug,
    year = "2009",
    address = "Singapore",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/W09-2902",
    pages = "9--16",
}

@InProceedings{nguyen_kan_2007,
author="Nguyen, Thuy Dung
and Kan, Min-Yen",
editor="Goh, Dion Hoe-Lian
and Cao, Tru Hoang
and S{\o}lvberg, Ingeborg Torvik
and Rasmussen, Edie",
title="Keyphrase Extraction in Scientific Publications",
booktitle="Asian Digital Libraries. Looking Back 10 Years and Forging New Frontiers",
year="2007",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="317--326",
isbn="978-3-540-77094-7"
}

@article{Gollapalli_Li_Yang_2017, 
title={Incorporating Expert Knowledge into Keyphrase Extraction}, volume={31}, url={https://ojs.aaai.org/index.php/AAAI/article/view/10986}, DOI={10.1609/aaai.v31i1.10986}, number={1}, journal={Proceedings of the AAAI Conference on Artificial Intelligence}, author={Gollapalli, Sujatha Das and Li, Xiao-li and Yang, Peng}, year={2017}, month={Feb.} }

@inproceedings{glove,
    title = "{G}lo{V}e: Global Vectors for Word Representation",
    author = "Pennington, Jeffrey  and
      Socher, Richard  and
      Manning, Christopher",
    booktitle = "Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing ({EMNLP})",
    month = oct,
    year = "2014",
    address = "Doha, Qatar",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/D14-1162",
    doi = "10.3115/v1/D14-1162",
    pages = "1532--1543",
}

@misc{word2vec,
  doi = {10.48550/ARXIV.1301.3781},
  
  url = {https://arxiv.org/abs/1301.3781},
  
  author = {Mikolov, Tomas and Chen, Kai and Corrado, Greg and Dean, Jeffrey},
  
  keywords = {Computation and Language (cs.CL), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Efficient Estimation of Word Representations in Vector Space},
  
  publisher = {arXiv},
  
  year = {2013},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{alzaidy_2019,
author = {Alzaidy, Rabah and Caragea, Cornelia and Giles, C. Lee},
title = {Bi-LSTM-CRF Sequence Labeling for Keyphrase Extraction from Scholarly Documents},
year = {2019},
isbn = {9781450366748},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3308558.3313642},
doi = {10.1145/3308558.3313642},
abstract = {In this paper, we address the keyphrase extraction problem as sequence labeling and propose a model that jointly exploits the complementary strengths of Conditional Random Fields that capture label dependencies through a transition parameter matrix consisting of the transition probabilities from one label to the neighboring label, and Bidirectional Long Short Term Memory networks that capture hidden semantics in text through the long distance dependencies. Our results on three datasets of scholarly documents show that the proposed model substantially outperforms strong baselines and previous approaches for keyphrase extraction.},
booktitle = {The World Wide Web Conference},
pages = {2551–2557},
numpages = {7},
keywords = {deep learning., Keyphrase extraction, sequence labeling},
location = {San Francisco, CA, USA},
series = {WWW '19}
}

@misc{attention-is-all-you-need,
  doi = {10.48550/ARXIV.1706.03762},
  
  url = {https://arxiv.org/abs/1706.03762},
  
  author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N. and Kaiser, Lukasz and Polosukhin, Illia},
  
  keywords = {Computation and Language (cs.CL), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Attention Is All You Need},
  
  publisher = {arXiv},
  
  year = {2017},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{tnt-kid,
	doi = {10.1017/s1351324921000127},
  
	url = {https://arxiv.org/abs/2003.09166},
  
	year = 2021,
	month = {jun},
  
	publisher = {Cambridge University Press ({CUP})},
  
	volume = {28},
  
	number = {4},
  
	pages = {409--448},
  
	author = {Matej Martinc and Bla{\v{z}
} {\v{S}}krlj and Senja Pollak},
  
	title = {{TNT}-{KID}: Transformer-based neural tagger for keyword identification},
  
	journal = {Natural Language Engineering}
}

@inproceedings{meng-etal-2017-deep,
    title = "Deep Keyphrase Generation",
    author = "Meng, Rui  and
      Zhao, Sanqiang  and
      Han, Shuguang  and
      He, Daqing  and
      Brusilovsky, Peter  and
      Chi, Yu",
    booktitle = "Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2017",
    address = "Vancouver, Canada",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/P17-1054",
    doi = "10.18653/v1/P17-1054",
    pages = "582--592",
    abstract = "Keyphrase provides highly-summative information that can be effectively used for understanding, organizing and retrieving text content. Though previous studies have provided many workable solutions for automated keyphrase extraction, they commonly divided the to-be-summarized content into multiple text chunks, then ranked and selected the most meaningful ones. These approaches could neither identify keyphrases that do not appear in the text, nor capture the real semantic meaning behind the text. We propose a generative model for keyphrase prediction with an encoder-decoder framework, which can effectively overcome the above drawbacks. We name it as \textit{deep keyphrase generation} since it attempts to capture the deep semantic meaning of the content with a deep learning method. Empirical analysis on six datasets demonstrates that our proposed model not only achieves a significant performance boost on extracting keyphrases that appear in the source text, but also can generate absent keyphrases based on the semantic meaning of the text. Code and dataset are available at \url{https://github.com/memray/seq2seq-keyphrase}.",
}

@inproceedings{ye-wang-2018-semi,
    title = "Semi-Supervised Learning for Neural Keyphrase Generation",
    author = "Ye, Hai  and
      Wang, Lu",
    booktitle = "Proceedings of the 2018 Conference on Empirical Methods in Natural Language Processing",
    month = oct # "-" # nov,
    year = "2018",
    address = "Brussels, Belgium",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/D18-1447",
    doi = "10.18653/v1/D18-1447",
    pages = "4142--4153",
    abstract = "We study the problem of generating keyphrases that summarize the key points for a given document. While sequence-to-sequence (seq2seq) models have achieved remarkable performance on this task (Meng et al., 2017), model training often relies on large amounts of labeled data, which is only applicable to resource-rich domains. In this paper, we propose semi-supervised keyphrase generation methods by leveraging both labeled data and large-scale unlabeled samples for learning. Two strategies are proposed. First, unlabeled documents are first tagged with synthetic keyphrases obtained from unsupervised keyphrase extraction methods or a self-learning algorithm, and then combined with labeled samples for training. Furthermore, we investigate a multi-task learning framework to jointly learn to generate keyphrases as well as the titles of the articles. Experimental results show that our semi-supervised learning-based methods outperform a state-of-the-art model trained with labeled data only.",
}

@article{Wu_Ma_Liu_Chen_Nie_2022, title={Fast and Constrained Absent Keyphrase Generation by Prompt-Based Learning}, volume={36}, url={https://ojs.aaai.org/index.php/AAAI/article/view/21402}, DOI={10.1609/aaai.v36i10.21402}, abstractNote={Generating absent keyphrases, which do not appear in the input document, is challenging in the keyphrase prediction task. Most previous works treat the problem as an autoregressive sequence-to-sequence generation task, which demonstrates promising results for generating grammatically correct and fluent absent keyphrases. However, such an end-to-end process with a complete data-driven manner is unconstrained, which is prone to generate keyphrases inconsistent with the input document. In addition, the existing autoregressive decoding method makes the generation of keyphrases must be done from left to right, leading to slow speed during inference. In this paper, we propose a constrained absent keyphrase generation method in a prompt-based learning fashion. Specifically, the prompt will be created firstly based on the keywords, which are defined as the overlapping words between absent keyphrase and document. Then, a mask-predict decoder is used to complete the absent keyphrase on the constraint of prompt. Experiments on keyphrase generation benchmarks have demonstrated the effectiveness of our approach. In addition, we evaluate the performance of constrained absent keyphrases generation from an information retrieval perspective. The result shows that our approach can generate more consistent keyphrases, which can improve document retrieval performance. What’s more, with a non-autoregressive decoding manner, our model can speed up the absent keyphrase generation by 8.67× compared with the autoregressive method.}, number={10}, journal={Proceedings of the AAAI Conference on Artificial Intelligence}, author={Wu, Huanqin and Ma, Baijiaxin and Liu, Wei and Chen, Tao and Nie, Dan}, year={2022}, month={Jun.}, pages={11495-11503} }

@misc{chen2018keyphrase,
      title={Keyphrase Generation with Correlation Constraints}, 
      author={Jun Chen and Xiaoming Zhang and Yu Wu and Zhao Yan and Zhoujun Li},
      year={2018},
      eprint={1808.07185},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{title-guided-kpg,
author = {Chen, Wang and Gao, Yifan and Zhang, Jiani and King, Irwin and Lyu, Michael R.},
title = {Title-Guided Encoding for Keyphrase Generation},
year = {2019},
isbn = {978-1-57735-809-1},
publisher = {AAAI Press},
url = {https://doi.org/10.1609/aaai.v33i01.33016268},
doi = {10.1609/aaai.v33i01.33016268},
abstract = {Keyphrase generation (KG) aims to generate a set of keyphrases given a document, which is a fundamental task in natural language processing (NLP). Most previous methods solve this problem in an extractive manner, while recently, several attempts are made under the generative setting using deep neural networks. However, the state-of-the-art generative methods simply treat the document title and the document main body equally, ignoring the leading role of the title to the overall document. To solve this problem, we introduce a new model called Title-Guided Network (TG-Net) for automatic keyphrase generation task based on the encoder-decoder architecture with two new features: (i) the title is additionally employed as a query-like input, and (ii) a title-guided encoder gathers the relevant information from the title to each word in the document. Experiments on a range of KG datasets demonstrate that our model outperforms the state-of-the-art models with a large margin, especially for documents with either very low or very high title length ratios.},
booktitle = {Proceedings of the Thirty-Third AAAI Conference on Artificial Intelligence and Thirty-First Innovative Applications of Artificial Intelligence Conference and Ninth AAAI Symposium on Educational Advances in Artificial Intelligence},
articleno = {769},
numpages = {8},
location = {Honolulu, Hawaii, USA},
series = {AAAI'19/IAAI'19/EAAI'19}
}

@inproceedings{wang-etal-2019-topic-aware,
    title = "Topic-Aware Neural Keyphrase Generation for Social Media Language",
    author = "Wang, Yue  and
      Li, Jing  and
      Chan, Hou Pong  and
      King, Irwin  and
      Lyu, Michael R.  and
      Shi, Shuming",
    booktitle = "Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2019",
    address = "Florence, Italy",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/P19-1240",
    doi = "10.18653/v1/P19-1240",
    pages = "2516--2526",
    abstract = "A huge volume of user-generated content is daily produced on social media. To facilitate automatic language understanding, we study keyphrase prediction, distilling salient information from massive posts. While most existing methods extract words from source posts to form keyphrases, we propose a sequence-to-sequence (seq2seq) based neural keyphrase generation framework, enabling absent keyphrases to be created. Moreover, our model, being topic-aware, allows joint modeling of corpus-level latent topic representations, which helps alleviate data sparsity widely exhibited in social media language. Experiments on three datasets collected from English and Chinese social media platforms show that our model significantly outperforms both extraction and generation models without exploiting latent topics. Further discussions show that our model learns meaningful topics, which interprets its superiority in social media keyphrase generation.",
}

@inproceedings{zhao-zhang-2019-incorporating,
    title = "Incorporating Linguistic Constraints into Keyphrase Generation",
    author = "Zhao, Jing  and
      Zhang, Yuxiang",
    booktitle = "Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2019",
    address = "Florence, Italy",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/P19-1515",
    doi = "10.18653/v1/P19-1515",
    pages = "5224--5233",
    abstract = "Keyphrases, that concisely describe the high-level topics discussed in a document, are very useful for a wide range of natural language processing tasks. Though existing keyphrase generation methods have achieved remarkable performance on this task, they generate many overlapping phrases (including sub-phrases or super-phrases) of keyphrases. In this paper, we propose the parallel Seq2Seq network with the coverage attention to alleviate the overlapping phrase problem. Specifically, we integrate the linguistic constraints of keyphrase into the basic Seq2Seq network on the source side, and employ the multi-task learning framework on the target side. In addition, in order to prevent from generating overlapping phrases of keyphrases with correct syntax, we introduce the coverage vector to keep track of the attention history and to decide whether the parts of source text have been covered by existing generated keyphrases. Experimental results show that our method can outperform the state-of-the-art CopyRNN on scientific datasets, and is also more effective in news domain.",
}

@misc{chan2019neural,
      title={Neural Keyphrase Generation via Reinforcement Learning with Adaptive Rewards}, 
      author={Hou Pong Chan and Wang Chen and Lu Wang and Irwin King},
      year={2019},
      eprint={1906.04106},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{swaminathan-etal-2020-preliminary,
    title = "A Preliminary Exploration of {GAN}s for Keyphrase Generation",
    author = "Swaminathan, Avinash  and
      Zhang, Haimin  and
      Mahata, Debanjan  and
      Gosangi, Rakesh  and
      Shah, Rajiv Ratn  and
      Stent, Amanda",
    booktitle = "Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.emnlp-main.645",
    doi = "10.18653/v1/2020.emnlp-main.645",
    pages = "8021--8030",
    abstract = "We introduce a new keyphrase generation approach using Generative Adversarial Networks (GANs). For a given document, the generator produces a sequence of keyphrases, and the discriminator distinguishes between human-curated and machine-generated keyphrases. We evaluated this approach on standard benchmark datasets. We observed that our model achieves state-of-the-art performance in the generation of abstractive keyphrases and is comparable to the best performing extractive techniques. Although we achieve promising results using GANs, they are not significantly better than the state-of-the-art generative models. To our knowledge, this is one of the first works that use GANs for keyphrase generation. We present a detailed analysis of our observations and expect that these findings would help other researchers to further study the use of GANs for the task of keyphrase generation.",
}

@inproceedings{chen-etal-2020-exclusive,
    title = "Exclusive Hierarchical Decoding for Deep Keyphrase Generation",
    author = "Chen, Wang  and
      Chan, Hou Pong  and
      Li, Piji  and
      King, Irwin",
    booktitle = "Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.acl-main.103",
    doi = "10.18653/v1/2020.acl-main.103",
    pages = "1095--1105",
    abstract = "Keyphrase generation (KG) aims to summarize the main ideas of a document into a set of keyphrases. A new setting is recently introduced into this problem, in which, given a document, the model needs to predict a set of keyphrases and simultaneously determine the appropriate number of keyphrases to produce. Previous work in this setting employs a sequential decoding process to generate keyphrases. However, such a decoding method ignores the intrinsic hierarchical compositionality existing in the keyphrase set of a document. Moreover, previous work tends to generate duplicated keyphrases, which wastes time and computing resources. To overcome these limitations, we propose an exclusive hierarchical decoding framework that includes a hierarchical decoding process and either a soft or a hard exclusion mechanism. The hierarchical decoding process is to explicitly model the hierarchical compositionality of a keyphrase set. Both the soft and the hard exclusion mechanisms keep track of previously-predicted keyphrases within a window size to enhance the diversity of the generated keyphrases. Extensive experiments on multiple KG benchmark datasets demonstrate the effectiveness of our method to generate less duplicated and more accurate keyphrases.",
}

@inproceedings{yuan-etal-2020-one,
    title = "One Size Does Not Fit All: Generating and Evaluating Variable Number of Keyphrases",
    author = "Yuan, Xingdi  and
      Wang, Tong  and
      Meng, Rui  and
      Thaker, Khushboo  and
      Brusilovsky, Peter  and
      He, Daqing  and
      Trischler, Adam",
    booktitle = "Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.acl-main.710",
    doi = "10.18653/v1/2020.acl-main.710",
    pages = "7961--7975",
    abstract = "Different texts shall by nature correspond to different number of keyphrases. This desideratum is largely missing from existing neural keyphrase generation models. In this study, we address this problem from both modeling and evaluation perspectives. We first propose a recurrent generative model that generates multiple keyphrases as delimiter-separated sequences. Generation diversity is further enhanced with two novel techniques by manipulating decoder hidden states. In contrast to previous approaches, our model is capable of generating diverse keyphrases and controlling number of outputs. We further propose two evaluation metrics tailored towards the variable-number generation. We also introduce a new dataset StackEx that expands beyond the only existing genre (i.e., academic writing) in keyphrase generation tasks. With both previous and new evaluation metrics, our model outperforms strong baselines on all datasets.",
}

@misc{zhao2021sgg,
      title={SGG: Learning to Select, Guide, and Generate for Keyphrase Generation}, 
      author={Jing Zhao and Junwei Bao and Yifan Wang and Youzheng Wu and Xiaodong He and Bowen Zhou},
      year={2021},
      eprint={2105.02544},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@article{Huang_Xu_Jiao_Zu_Zhang_2021, title={Adaptive Beam Search Decoding for Discrete Keyphrase Generation}, volume={35}, url={https://ojs.aaai.org/index.php/AAAI/article/view/17546}, DOI={10.1609/aaai.v35i14.17546}, abstractNote={Keyphrase Generation compresses a document into some highly-summative phrases, which is an important task in natural language processing. Most state-of-the-art adopt greedy search or beam search decoding methods. These two decoding methods generate a large number of duplicated keyphrases and are time-consuming. Moreover, beam search only predicts a fixed number of keyphrases for different documents. In this paper, we propose an adaptive generation model-AdaGM, which is mainly inspired by the importance of the first words in keyphrase generation. In AdaGM, a novel reset state training mechanism is proposed to maximize the difference in the predicted first words. To ensure the discreteness and get an appropriate number of keyphrases according to the content of the document adaptively, we equip beam search with a highly effective filter mechanism. Experiments on five public datasets demonstrate the proposed model can generate marginally less duplicated and more accurate keyphrases. The codes of AdaGM are available at: https://github.com/huangxiaolist/adaGM.}, number={14}, journal={Proceedings of the AAAI Conference on Artificial Intelligence}, author={Huang, Xiaoli and Xu, Tongge and Jiao, Lvan and Zu, Yueran and Zhang, Youmin}, year={2021}, month={May}, pages={13082-13089} }

@inproceedings{ye-etal-2021-one2set,
    title = "{O}ne2{S}et: {G}enerating Diverse Keyphrases as a Set",
    author = "Ye, Jiacheng  and
      Gui, Tao  and
      Luo, Yichao  and
      Xu, Yige  and
      Zhang, Qi",
    booktitle = "Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)",
    month = aug,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.acl-long.354",
    doi = "10.18653/v1/2021.acl-long.354",
    pages = "4598--4608",
    abstract = "Recently, the sequence-to-sequence models have made remarkable progress on the task of keyphrase generation (KG) by concatenating multiple keyphrases in a predefined order as a target sequence during training. However, the keyphrases are inherently an unordered set rather than an ordered sequence. Imposing a predefined order will introduce wrong bias during training, which can highly penalize shifts in the order between keyphrases. In this work, we propose a new training paradigm One2Set without predefining an order to concatenate the keyphrases. To fit this paradigm, we propose a novel model that utilizes a fixed set of learned control codes as conditions to generate a set of keyphrases in parallel. To solve the problem that there is no correspondence between each prediction and target during training, we propose a K-step label assignment mechanism via bipartite matching, which greatly increases the diversity and reduces the repetition rate of generated keyphrases. The experimental results on multiple benchmarks demonstrate that our approach significantly outperforms the state-of-the-art methods.",
}

@article{Chen2019AnIA,
  title={An Integrated Approach for Keyphrase Generation via Exploring the Power of Retrieval and Extraction},
  author={Wang Chen and Hou Pong Chan and Piji Li and Lidong Bing and Irwin King},
  journal={ArXiv},
  year={2019},
  volume={abs/1904.03454}
}

@inproceedings{ahmad-etal-2021-select,
    title = "Select, Extract and Generate: Neural Keyphrase Generation with Layer-wise Coverage Attention",
    author = "Ahmad, Wasi  and
      Bai, Xiao  and
      Lee, Soomin  and
      Chang, Kai-Wei",
    booktitle = "Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)",
    month = aug,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.acl-long.111",
    doi = "10.18653/v1/2021.acl-long.111",
    pages = "1389--1404",
    abstract = "Natural language processing techniques have demonstrated promising results in keyphrase generation. However, one of the major challenges in \textit{neural} keyphrase generation is processing long documents using deep neural networks. Generally, documents are truncated before given as inputs to neural networks. Consequently, the models may miss essential points conveyed in the target document. To overcome this limitation, we propose \textit{SEG-Net}, a neural keyphrase generation model that is composed of two major components, (1) a selector that selects the salient sentences in a document and (2) an extractor-generator that jointly extracts and generates keyphrases from the selected sentences. SEG-Net uses Transformer, a self-attentive architecture, as the basic building block with a novel \textit{layer-wise} coverage attention to summarize most of the points discussed in the document. The experimental results on seven keyphrase generation benchmarks from scientific and web documents demonstrate that SEG-Net outperforms the state-of-the-art neural generative methods by a large margin.",
}

@misc{wu2021unikeyphrase,
      title={UniKeyphrase: A Unified Extraction and Generation Framework for Keyphrase Prediction}, 
      author={Huanqin Wu and Wei Liu and Lei Li and Dan Nie and Tao Chen and Feng Zhang and Di Wang},
      year={2021},
      eprint={2106.04847},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{NIPS2017_d5e2c0ad,
 author = {Christiano, Paul F and Leike, Jan and Brown, Tom and Martic, Miljan and Legg, Shane and Amodei, Dario},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {I. Guyon and U. Von Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Deep Reinforcement Learning from Human Preferences},
 url = {https://proceedings.neurips.cc/paper_files/paper/2017/file/d5e2c0adad503c91f91df240d0cd4e49-Paper.pdf},
 volume = {30},
 year = {2017}
}

@misc{ibarz2018reward,
      title={Reward learning from human preferences and demonstrations in Atari}, 
      author={Borja Ibarz and Jan Leike and Tobias Pohlen and Geoffrey Irving and Shane Legg and Dario Amodei},
      year={2018},
      eprint={1811.06521},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{ziegler2020finetuning,
      title={Fine-Tuning Language Models from Human Preferences}, 
      author={Daniel M. Ziegler and Nisan Stiennon and Jeffrey Wu and Tom B. Brown and Alec Radford and Dario Amodei and Paul Christiano and Geoffrey Irving},
      year={2020},
      eprint={1909.08593},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{stiennon2022learning,
      title={Learning to summarize from human feedback}, 
      author={Nisan Stiennon and Long Ouyang and Jeff Wu and Daniel M. Ziegler and Ryan Lowe and Chelsea Voss and Alec Radford and Dario Amodei and Paul Christiano},
      year={2022},
      eprint={2009.01325},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{böhm2019better,
      title={Better Rewards Yield Better Summaries: Learning to Summarise Without References}, 
      author={Florian Böhm and Yang Gao and Christian M. Meyer and Ori Shapira and Ido Dagan and Iryna Gurevych},
      year={2019},
      eprint={1909.01214},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{wu2021recursively,
      title={Recursively Summarizing Books with Human Feedback}, 
      author={Jeff Wu and Long Ouyang and Daniel M. Ziegler and Nisan Stiennon and Ryan Lowe and Jan Leike and Paul Christiano},
      year={2021},
      eprint={2109.10862},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{jaques2019way,
      title={Way Off-Policy Batch Deep Reinforcement Learning of Implicit Human Preferences in Dialog}, 
      author={Natasha Jaques and Asma Ghandeharioun and Judy Hanwen Shen and Craig Ferguson and Agata Lapedriza and Noah Jones and Shixiang Gu and Rosalind Picard},
      year={2019},
      eprint={1907.00456},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{Kreutzer2018CanNM,
  title={Can Neural Machine Translation be Improved with User Feedback?},
  author={Julia Kreutzer and Shahram Khadivi and Evgeny Matusov and Stefan Riezler},
  booktitle={North American Chapter of the Association for Computational Linguistics},
  year={2018}
}

@inproceedings{lawrence-riezler-2018-improving,
    title = "Improving a Neural Semantic Parser by Counterfactual Learning from Human Bandit Feedback",
    author = "Lawrence, Carolin  and
      Riezler, Stefan",
    booktitle = "Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2018",
    address = "Melbourne, Australia",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/P18-1169",
    doi = "10.18653/v1/P18-1169",
    pages = "1820--1830",
    abstract = "Counterfactual learning from human bandit feedback describes a scenario where user feedback on the quality of outputs of a historic system is logged and used to improve a target system. We show how to apply this learning framework to neural semantic parsing. From a machine learning perspective, the key challenge lies in a proper reweighting of the estimator so as to avoid known degeneracies in counterfactual learning, while still being applicable to stochastic gradient optimization. To conduct experiments with human users, we devise an easy-to-use interface to collect human feedback on semantic parses. Our work is the first to show that semantic parsers can be improved significantly by counterfactual learning from logged human feedback data.",
}

@misc{zhou2020learning,
      title={Learning to Compare for Better Training and Evaluation of Open Domain Natural Language Generation Models}, 
      author={Wangchunshu Zhou and Ke Xu},
      year={2020},
      eprint={2002.05058},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{cho2019coherent,
      title={Towards Coherent and Cohesive Long-form Text Generation}, 
      author={Woon Sang Cho and Pengchuan Zhang and Yizhe Zhang and Xiujun Li and Michel Galley and Chris Brockett and Mengdi Wang and Jianfeng Gao},
      year={2019},
      eprint={1811.00511},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@article{Perez2019FindingGE,
  title={Finding Generalizable Evidence by Learning to Convince Q\&A Models},
  author={Ethan Perez and Siddharth Karamcheti and Rob Fergus and Jason Weston and Douwe Kiela and Kyunghyun Cho},
  journal={ArXiv},
  year={2019},
  volume={abs/1909.05863}
}

@misc{madaan2023memoryassisted,
      title={Memory-assisted prompt editing to improve GPT-3 after deployment}, 
      author={Aman Madaan and Niket Tandon and Peter Clark and Yiming Yang},
      year={2023},
      eprint={2201.06009},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{howard-ruder-2018-universal,
    title = "Universal Language Model Fine-tuning for Text Classification",
    author = "Howard, Jeremy  and
      Ruder, Sebastian",
    booktitle = "Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2018",
    address = "Melbourne, Australia",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/P18-1031",
    doi = "10.18653/v1/P18-1031",
    pages = "328--339",
    abstract = "Inductive transfer learning has greatly impacted computer vision, but existing approaches in NLP still require task-specific modifications and training from scratch. We propose Universal Language Model Fine-tuning (ULMFiT), an effective transfer learning method that can be applied to any task in NLP, and introduce techniques that are key for fine-tuning a language model. Our method significantly outperforms the state-of-the-art on six text classification tasks, reducing the error by 18-24{\%} on the majority of datasets. Furthermore, with only 100 labeled examples, it matches the performance of training from scratch on 100 times more data. We open-source our pretrained models and code.",
}

@misc{wang2020superglue,
      title={SuperGLUE: A Stickier Benchmark for General-Purpose Language Understanding Systems}, 
      author={Alex Wang and Yada Pruksachatkun and Nikita Nangia and Amanpreet Singh and Julian Michael and Felix Hill and Omer Levy and Samuel R. Bowman},
      year={2020},
      eprint={1905.00537},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{devlin2019bert,
      title={BERT: Pre-training of Deep Bidirectional Transformers for Language Understanding}, 
      author={Jacob Devlin and Ming-Wei Chang and Kenton Lee and Kristina Toutanova},
      year={2019},
      eprint={1810.04805},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{dong2019unified,
      title={Unified Language Model Pre-training for Natural Language Understanding and Generation}, 
      author={Li Dong and Nan Yang and Wenhui Wang and Furu Wei and Xiaodong Liu and Yu Wang and Jianfeng Gao and Ming Zhou and Hsiao-Wuen Hon},
      year={2019},
      eprint={1905.03197},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{mccann2018natural,
      title={The Natural Language Decathlon: Multitask Learning as Question Answering}, 
      author={Bryan McCann and Nitish Shirish Keskar and Caiming Xiong and Richard Socher},
      year={2018},
      eprint={1806.08730},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{keskar2019unifying,
      title={Unifying Question Answering, Text Classification, and Regression via Span Extraction}, 
      author={Nitish Shirish Keskar and Bryan McCann and Caiming Xiong and Richard Socher},
      year={2019},
      eprint={1904.09286},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{hendy2023good,
      title={How Good Are GPT Models at Machine Translation? A Comprehensive Evaluation}, 
      author={Amr Hendy and Mohamed Abdelrehim and Amr Sharaf and Vikas Raunak and Mohamed Gabr and Hitokazu Matsushita and Young Jin Kim and Mohamed Afify and Hany Hassan Awadalla},
      year={2023},
      eprint={2302.09210},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@inproceedings{kim_2010,
author = {Kim, Su Nam and Medelyan, Olena and Kan, Min-Yen and Baldwin, Timothy},
title = {SemEval-2010 Task 5: Automatic Keyphrase Extraction from Scientific Articles},
year = {2010},
publisher = {Association for Computational Linguistics},
address = {USA},
abstract = {This paper describes Task 5 of the Workshop on Semantic Evaluation 2010 (SemEval-2010). Systems are to automatically assign keyphrases or keywords to given scientific articles. The participating systems were evaluated by matching their extracted keyphrases against manually assigned ones. We present the overall ranking of the submitted systems and discuss our findings to suggest future directions for this task.},
booktitle = {Proceedings of the 5th International Workshop on Semantic Evaluation},
pages = {21–26},
numpages = {6},
location = {Los Angeles, California},
series = {SemEval '10}
}

@InProceedings{nguyen_kan_2007,
author="Nguyen, Thuy Dung
and Kan, Min-Yen",
editor="Goh, Dion Hoe-Lian
and Cao, Tru Hoang
and S{\o}lvberg, Ingeborg Torvik
and Rasmussen, Edie",
title="Keyphrase Extraction in Scientific Publications",
booktitle="Asian Digital Libraries. Looking Back 10 Years and Forging New Frontiers",
year="2007",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="317--326",
isbn="978-3-540-77094-7"
}

@inproceedings{hulth2003,
author = {Hulth, Anette},
title = {Improved Automatic Keyword Extraction given More Linguistic Knowledge},
year = {2003},
publisher = {Association for Computational Linguistics},
address = {USA},
url = {https://doi.org/10.3115/1119355.1119383},
doi = {10.3115/1119355.1119383},
booktitle = {Proceedings of the 2003 Conference on Empirical Methods in Natural Language Processing},
pages = {216–223},
numpages = {8},
series = {EMNLP '03}
}

@inproceedings{duc2001,
author = {Wan, Xiaojun and Xiao, Jianguo},
title = {Single Document Keyphrase Extraction Using Neighborhood Knowledge},
year = {2008},
isbn = {9781577353683},
publisher = {AAAI Press},
abstract = {Existing methods for single document keyphrase extraction usually make use of only the information contained in the specified document. This paper proposes to use a small number of nearest neighbor documents to provide more knowledge to improve single document keyphrase extraction. A specified document is expanded to a small document set by adding a few neighbor documents close to the document, and the graph-based ranking algorithm is then applied on the expanded document set to make use of both the local information in the specified document and the global information in the neighbor documents. Experimental results demonstrate the good effectiveness and robustness of our proposed approach.},
booktitle = {Proceedings of the 23rd National Conference on Artificial Intelligence - Volume 2},
pages = {855–860},
numpages = {6},
location = {Chicago, Illinois},
series = {AAAI'08}
}

@misc{gallina2019kptimes,
      title={KPTimes: A Large-Scale Dataset for Keyphrase Generation on News Documents}, 
      author={Ygor Gallina and Florian Boudin and Béatrice Daille},
      year={2019},
      eprint={1911.12559},
      archivePrefix={arXiv},
      primaryClass={cs.IR}
}

@misc{song2023chatgpt,
      title={Is ChatGPT A Good Keyphrase Generator? A Preliminary Study}, 
      author={Mingyang Song and Haiyun Jiang and Shuming Shi and Songfang Yao and Shilong Lu and Yi Feng and Huafeng Liu and Liping Jing},
      year={2023},
      eprint={2303.13001},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@article{query-based-kpe,
	doi = {10.32473/flairs.v35i.130737},
  
	url = {https://doi.org/10.32473\%2Fflairs.v35i.130737},
  
	year = 2022,
	month = {may},
  
	publisher = {University of Florida George A Smathers Libraries},
  
	volume = {35},
  
	author = {Martin Do{\v{c}}ekal and Pavel Smr{\v{z}}},
  
	title = {Query-Based Keyphrase Extraction from Long Documents},
  
	journal = {The International {FLAIRS} Conference Proceedings}
}

@article{mahata2022ldkp,
  title={LDKP: A Dataset for Identifying Keyphrases from Long Scientific Documents},
  author={Mahata, Debanjan and Agarwal, Naveen and Gautam, Dibya and Kumar, Amardeep and Parekh, Swapnil and Singla, Yaman Kumar and Acharya, Anish and Shah, Rajiv Ratn},
  journal={arXiv preprint arXiv:2203.15349},
  year={2022}
}

@misc{garg2022keyphrase,
      title={Keyphrase Generation Beyond the Boundaries of Title and Abstract}, 
      author={Krishna Garg and Jishnu Ray Chowdhury and Cornelia Caragea},
      year={2022},
      eprint={2112.06776},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{martinezcruz2023,
      title={Enhancing Keyphrase Extraction from Long Scientific Documents using Graph Embeddings}, 
      author={Roberto Martínez-Cruz and Debanjan Mahata and Alvaro J. López-López and José Portela},
      year={2023},
      eprint={2305.09316},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}
